ProtoCon: Pseudo-label Refinement via Online Clustering and Prototypical Consistency for Efficient Semi-supervised Learning

Confidence-based pseudo-labeling is among the dominant approaches in semi-supervised learning (SSL). It relies on including high-confidence predictions made on unlabeled data as additional targets to train the model. We propose ProtoCon, a novel SSL method aimed at the less-explored label-scarce SSL where such methods usually underperform. ProtoCon refines the pseudo-labels by leveraging their nearest neighbours' information. The neighbours are identified as the training proceeds using an online clustering approach operating in an embedding space trained via a prototypical loss to encourage well-formed clusters. The online nature of ProtoCon allows it to utilise the label history of the entire dataset in one training cycle to refine labels in the following cycle without the need to store image embeddings. Hence, it can seamlessly scale to larger datasets at a low cost. Finally, ProtoCon addresses the poor training signal in the initial phase of training (due to fewer confident predictions) by introducing an auxiliary self-supervised loss. It delivers significant gains and faster convergence over state-of-the-art across 5 datasets, including CIFARs, ImageNet and DomainNet.

==> tables/supplements_cifar_and_mini_results.tex <==
\begin{table*}[h!]
\centering
\caption{\small{Complete Tab.~\ref{tab:cifar_results} results. CIFAR and Mini-ImageNet accuracy for different amounts of labeled samples averaged over 5 different splits. All results are produced using the same codebase and same splits.}}
\label{tab:cifar_results_supp}
\scalebox{0.77}{
\begin{tabular}{llccclccclcc}
\toprule[0.15em]
 &  & \multicolumn{3}{c}{\bf CIFAR-10} &  & \multicolumn{3}{c}{\bf CIFAR-100} &  & \multicolumn{2}{c}{\bf Mini-ImageNet} \\ \cline{3-5} \cline{7-9} \cline{11-12} 
Total labeled samples &  & 20 & 40 & 80 &  & 200 & 400 & 800 &  & 400 & 1000 \\ \midrule[0.15em]
FixMatch~\cite{Sohn_fixmatch20} &  & 82.32$\pm$9.77 & 86.29$\pm$4.50 & 92.06$\pm$0.88 &  & 35.37$\pm$5.68 & 51.15$\pm$1.75 & 61.32$\pm$0.92 &  & 17.18$\pm$6.22 & 39.03$\pm$3.99 \\
FixMatch + DA~\cite{Sohn_fixmatch20, Berthelot_RemixMatch19} &  & 83.84$\pm$8.35 & 86.98$\pm$3.40 & 92.29$\pm$0.86 &  & 41.28$\pm$6.03 & 52.65$\pm$2.32 & 62.12$\pm$0.79 &  & 19.40$\pm$5.87 & 40.92$\pm$4.71\\
CoMatch~\cite{li2021comatch} &  & 87.37$\pm$8.47 & 93.09$\pm$1.39 & 93.97$\pm$0.62 &  & 47.92$\pm$4.83 & 58.17$\pm$3.52 & \bf 66.15$\pm$0.71 &  & 21.29$\pm$6.19 & 40.98$\pm$3.52\\
FixMatch + DB~\cite{wang2022debiased} &  & 89.02$\pm$6.37 & 94.60 $\pm$1.31 & 95.60 $\pm$0.12 &  & 46.36$\pm$5.05 & 57.88$\pm$3.34 & 64.84$\pm$0.85 &  & 27.37$\pm$7.01 & 41.05$\pm$3.34\\
\midrule[0.15em]
\rowcolor{_fbteal3}
\putouralg  &  & \bf 90.51$\pm$4.02 & \bf 95.20$\pm$1.8 & \bf 96.11$\pm$0.20 &  & \bf 48.25$\pm$4.87 & \bf 59.53$\pm$2.94 & 65.91$\pm$0.57 &  & \bf 29.15$\pm$6.98 & \bf 45.83$\pm$4.15\\
\emph{delta against best baseline}  &  & {\color{darkgreen} +1.49} & {\color{darkgreen} +0.60} & {\color{darkgreen} +0.51} &  & {\color{darkgreen} +0.33} & {\color{darkgreen} +1.36} & {\color{darkred} -0.24} &  & {\color{darkgreen} +1.78} & {\color{darkgreen} +4.78}\\
\bottomrule[0.15em]
\end{tabular}%
}
% \vspace{-2mm}

\end{table*}

==> tables/supplements_domainnet_results.tex <==
\begin{table}[h!]
\centering
\caption{\small{Complete Tab.~\ref{tab:domain_results} results. DomainNet accuracy for 2, 4, and 8 labels per class.}}
\label{tab:domain_results_supp}
\scalebox{0.7}{
\begin{tabular}{llccclccc}
\toprule[0.15em]
 &  & \multicolumn{3}{c}{\bf Clipart} &  & \multicolumn{3}{c}{\bf Sketch} \\ \cline{3-5} \cline{7-9} 
Total labeled samples &  & 690 & 1380 & 2760 &  & 690 & 1380 & 2760 \\ \midrule[0.15em]
FixMatch~\cite{Sohn_fixmatch20} &  & 30.21 & 41.21 & 51.29 &  & 12.73 & 21.65 & 33.07 \\
CoMatch~\cite{li2021comatch} &  & 35.49 & 48.62 & 54.98 &  & 24.30 & 33.71 & 41.02 \\
FixMatch + DB~\cite{wang2022debiased} &  & 38.97 & 51.44 & 58.31 &  & 25.34 & 35.58 & 43.98 \\
\midrule[0.15em]
\rowcolor{_fbteal3}
\putouralg  &  & \bf 43.72 & \bf 55.66 & \bf 61.32 &  & \bf 33.94 & \bf 43.51 & \bf 50.88 \\
\emph{delta}  &  & {\color{darkgreen} +4.75} & {\color{darkgreen} +4.22} & {\color{darkgreen} +3.01} &  & {\color{darkgreen} +8.60} & {\color{darkgreen} +7.93} & {\color{darkgreen} +6.90} \\
\bottomrule[0.15em]
\end{tabular}%
}
% \vspace{-2mm}

\end{table}

==> tables/supplements_imagenet_results.tex <==
\begin{table}[h]
\centering
\caption{\small Complete Tab.~\ref{tab:imagenet_results} results. SSL results on ImageNet with different percentage of labels. $\dagger$ denotes results produced by our codebase. Other results are reported as appearing in the cited work. }
\label{tab:imagenet_results_supp}
% \vspace{-2mm}
\setlength{\tabcolsep}{2pt}
\scalebox{0.9}{
    \begin{tabular}{l r c c c c}
        % & & & \multicolumn{2}{c}{\small Top 1}\\
        \small Method & \small Pre. & \small Epochs & \small 0.2\% & \small 1\% & \small 10\% \\\toprule [0.15em]
        Supervised & \xmark & 300 & -- & 25.4 & 56.4\\ \midrule[0.15em]
        \multicolumn{4}{l}{\footnotesize\itshape Representation learning methods:}\\[1mm]
        SwAV~\cite{caron2020unsupervised} & \cmark & 800 & -- & 53.9 & 70.2 \\
        SimCLRv2++ ~\cite{chen2020big} & \cmark & 1200 & --  & 60.0 & 70.5 \\
        DINO~\cite{caron2021emerging} & \cmark & 300 & -- & 55.1 & 67.8 \\
        PAWS++ ~\cite{assran2021semi} & \cmark & 300 & --  & 66.5 & \textbf{75.5} \\\midrule[0.15em]
        \multicolumn{4}{l}{\footnotesize\itshape PL \& consistency methods:}\\[1mm]
        MPL~\cite{pham2021meta} & \xmark & 800 & -- & $65.3^\dagger$ & 73.9 \\
        CoMatch~\cite{li2021comatch} & \xmark & 400 & $44.3^\dagger$ & 66.0 & 73.6 \\
        FixMatch~\cite{Sohn_fixmatch20} & \xmark & 300 & -- & 51.2 & 71.5 \\
        FMatch + DA~\cite{Sohn_fixmatch20, Berthelot_RemixMatch19} & \xmark & 300 & $41.1^\dagger$ & 53.4 & $71.5^\dagger$ \\
        FMatch + EMAN~\cite{cai2021exponential} & \cmark & 850 & 43.6 & 60.9 & 72.6 \\
        FMatch + DB~\cite{wang2022debiased} & \xmark & 300 & $45.8^\dagger$ & $63.0^\dagger$ & $71.7^\dagger$ \\
        FMatch + DB + EMAN~\cite{wang2022debiased} & \cmark & 850 & 47.9 & 63.1 & $72.8^\dagger$ \\
        \midrule[0.15em]
        \rowcolor{_fbteal3}
        \putouralg & \xmark & 300 & 47.8 & 65.6 & 73.1 \\
        \rowcolor{_fbteal3}
        \putouralg + EMAN~\cite{cai2021exponential} & \cmark & 850 & \bf 50.1 & \bf 67.2 &  73.5 \\
        \emph{delta against best baseline} &  &  & {\color{darkgreen} +2.2} & {\color{darkgreen} +0.7} &  {\color{darkred} -2.0} \\
        \bottomrule[0.15em]
    \end{tabular}}
\vspace*{0em}
\end{table} 
